Illuminating Diverse Neural Cellular Automata for Level Generation

We present a method of generating diverse collections of neural cellular automata (NCA) to design video game levels. While NCAs have so far only been trained via supervised learning, we present a quality diversity (QD) approach to generating a collection of NCA level generators. By framing the problem as a QD problem, our approach can train diverse level generators, whose output levels vary based on aesthetic or functional criteria. To efficiently generate NCAs, we train generators via Covariance Matrix Adaptation MAP-Elites (CMA-ME), a quality diversity algorithm which specializes in continuous search spaces. We apply our new method to generate level generators for several 2D tile-based games: a maze game, Sokoban, and Zelda. Our results show that CMA-ME can generate small NCAs that are diverse yet capable, often satisfying complex solvability criteria for deterministic agents. We compare against a Compositional Pattern-Producing Network (CPPN) baseline trained to produce diverse collections of generators and show that the NCA representation yields a better exploration of level-space.

==> Illuminating Diverse NCA Level Generators (arxiv) 2/tables/cross_eval.tex <==
\begin{table*}
\centering
\caption{\textbf{Hyperparameter ablations in the maze domain on the NCA model, with exploration along measures of path-length and symmetry.}}
\label{tbl:cross_eval}
\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
    &    &           &     & \multicolumn{3}{c|}{Training} & \multicolumn{3}{c|}{Evaluation} \\
\cline{5-10}
    &    &           &     &            archive size &             QD score & \begin{tabular}[c]{@{}l@{}}generator\\ diversity\end{tabular} &            archive size &             QD score & \begin{tabular}[c]{@{}l@{}}generator\\ diversity\end{tabular} \\
\textbf{model} & \textbf{\begin{tabular}[c]{@{}l@{}}batch\\ size\end{tabular}} & \textbf{latents} & \textbf{\begin{tabular}[c]{@{}l@{}}num.\\ steps\end{tabular}} &                         &                      &                                                               &                         &                      &                                                               \\
\hline
\multirow{8}{*}{\textbf{NCA}} & \multirow{4}{*}{\textbf{10}} & \multirow{2}{*}{\textbf{Fix}} & \textbf{50 } &           4,584 ± 456.2 &           860 ± 57.1 &                                         0.37 ± 0.0 &           3,122 ± 289.9 &           386 ± 36.6 &                                         0.36 ± 0.0 \\
    &    &           & \textbf{100} &           6,804 ± 342.8 &           849 ± 42.4 &                                         0.37 ± 0.0 &           3,162 ± 286.9 &           392 ± 35.5 &                                         0.37 ± 0.0 \\
\cline{3-10}
    &    & \multirow{2}{*}{\textbf{Re-sample}} & \textbf{50 } &           6,442 ± 359.1 &           797 ± 42.7 &                                         0.35 ± 0.0 &           3,396 ± 207.6 &           417 ± 24.4 &                                         0.34 ± 0.0 \\
    &    &           & \textbf{100} &           6,560 ± 295.5 &           816 ± 38.3 &                                         0.35 ± 0.0 &           3,477 ± 186.3 &           430 ± 24.0 &                                         0.35 ± 0.0 \\
\cline{2-10}
\cline{3-10}
    & \multirow{4}{*}{\textbf{20}} & \multirow{2}{*}{\textbf{Fix}} & \textbf{50 } &           6,650 ± 491.1 &           826 ± 62.4 &                                         0.35 ± 0.0 &           3,458 ± 454.2 &           428 ± 56.7 &                                         0.35 ± 0.0 \\
    &    &           & \textbf{100} &  \textbf{6,938} ± 365.4 &  \textbf{863} ± 48.3 &                                         0.37 ± 0.0 &           3,596 ± 278.8 &           446 ± 33.8 &                                         0.35 ± 0.0 \\
\cline{3-10}
    &    & \multirow{2}{*}{\textbf{Re-sample}} & \textbf{50 } &           6,458 ± 618.7 &           798 ± 82.0 &                                         0.34 ± 0.0 &           3,683 ± 385.7 &           454 ± 50.9 &                                         0.34 ± 0.0 \\
    &    &           & \textbf{100} &           6,604 ± 269.8 &           817 ± 36.3 &                                \textbf{0.37} ± 0.0 &  \textbf{3,747} ± 207.4 &  \textbf{462} ± 28.1 &                                \textbf{0.37} ± 0.0 \\
\hline
\end{tabular}
\end{table*}

==> Illuminating Diverse NCA Level Generators (arxiv) 2/tables/cross_eval_models.tex <==
\begin{table*}
\centering
\caption{Neural architecture performance on maze-generation task, with exploration along measures of path-length and symetry. NCAs outperform Decoders, as well as indirect-encoding and generative, mutable and fixed-topology CPPNs, in terms of archive size and Quality Diversity score during training, and maintain the highest QD score during evaluation. Intra-generator diversity is significantly higher among NCAs during both training and evaluation. Note that non-generative (indirect-encoding) CPPNs are not evaluated on new latent seeds, since they take only $(x, y)$ coordinates as input.}
\label{tbl:cross_eval_models}
\label{{'tbl:cross_eval'}}
\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
         &    & \multicolumn{3}{c|}{Training} & \multicolumn{3}{c|}{Evaluation} \\
\cline{3-8}
         &    &            archive size &             QD score & \begin{tabular}[c]{@{}l@{}}generator\\ diversity\end{tabular} &            archive size &             QD score & \begin{tabular}[c]{@{}l@{}}generator\\ diversity\end{tabular} \\
\textbf{model} & \textbf{\begin{tabular}[c]{@{}l@{}}num.\\ steps\end{tabular}} &                         &                      &                                                               &                         &                      &                                                               \\
\hline
%\textbf{AttentionNCA} & \textbf{50} &           5,277 ± 426.3 &           648 ± 51.7 &                                         0.09 ± 0.0 &           3,890 ± 330.0 &           479 ± 40.5 &                                         0.08 ± 0.0 \\
\textbf{CPPN} & \textbf{1 } &           4,959 ± 893.1 &           424 ± 35.2 &                                          --- &  --- &           --- &                                         --- \\
\textbf{SinCPPN} & \textbf{1 } &            1,930 ± 13.1 &            233 ± 1.6 &                                          --- &            --- &            --- &                                         --- \\
\textbf{Decoder} & \textbf{1 } &           3,502 ± 167.8 &           429 ± 21.2 &                                \textbf{1.14} ± 0.1 &              828 ± 52.6 &             94 ± 6.4 &                                \textbf{1.29} ± 0.0 \\
% \textbf{DeepDecoder} & \textbf{1 } &           3,443 ± 287.5 &           435 ± 36.6 &                                         0.32 ± 0.0 &           2,043 ± 145.1 &           258 ± 18.4 &                                         0.37 ± 0.0 \\
\textbf{GenCPPN} & \textbf{1 } &           2,003 ± 142.6 &           250 ± 17.2 &                                         0.32 ± 0.0 &            1,078 ± 61.1 &            134 ± 7.5 &                                         0.35 ± 0.0 \\
\textbf{GenSinCPPN} & \textbf{1 } &               619 ± 6.4 &             71 ± 0.7 &                                         0.33 ± 0.0 &               220 ± 6.5 &             25 ± 0.7 &                                         0.33 ± 0.0 \\
\textbf{NCA} & \textbf{50} &           4,584 ± 456.2 &           860 ± 57.1 &                                         0.37 ± 0.0 &           3,122 ± 289.9 &           386 ± 36.6 &                                         0.36 ± 0.0 \\
\textbf{AuxNCA} & \textbf{50} &  \textbf{7,118} ± 802.0 &  \textbf{910} ± 95.0 &                                         0.23 ± 0.1 &           \textbf{4,035} ± 596.9 &  \textbf{501} ± 76.3 &                                         0.23 ± 0.1 \\
\hline
\end{tabular}
\end{table*}
